Can the Parts Fool the Test? Counterfactual Pairing Cycles for Relational OOD

Relational out-of-distribution errors are easy to describe and hard to evaluate cleanly. An image may be natural, a caption may be fluent, and all mentioned objects may be common, yet the caption may describe the wrong relation in the image. Many evaluations intended to test this behavior can be solved without checking the pairing at all, because negatives differ in caption style, template, length, object frequency, or image statistics. We propose counterfactual pairing cycles, a blocked evaluation primitive that reuses the same two images and the same two captions on both sides of the comparison, changing only which image is paired with which caption. This makes image-only, text-only, and additive component shortcuts cancel exactly in finite samples. The same contrast also gives a training loss for relational outlier exposure and a diagnostic for bilinear vision-language scores. Across synthetic controls, GQA, and COCO, cycles separate coarse image-caption matching from directional role-binding failures, while also identifying geometric size relations that remain strongly visible in global features. In a shortcut-contaminated COCO outlier-exposure stress test, a model selected by a near-perfect shortcut validation AUROC retains substantial relational signal but remains below cycle training on exact cycles; cycle training improves CycleAcc from 0.882 to 0.927. The main lesson is simple: to test whether a model understands a pairing, the benchmark should keep the parts fixed, change the pairing, and ask only about coupling. The official implementation is available online.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}  

\begin{enumerate}  
	
	\item {\bf Claims}  
	\item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The abstract and introduction state the main contributions: counterfactual pairing cycles, additive-shortcut cancellation, cycle loss, bilinear diagnostics, and experiments on synthetic controls, GQA, and COCO. The claims are matched to the theory and experiments, and the paper states that cycle success indicates coupling sensitivity rather than full semantic understanding.  
	
	\item {\bf Limitations}  
	\item[] Question: Does the paper discuss the limitations of the work performed by the authors?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The appendix includes a Limitations section discussing remaining non-additive shortcuts, annotation and geometry noise, and the focus on frozen CLIP ViT-B/32 features and bilinear probes.  
	
	\item {\bf Theory assumptions and proofs}  
	\item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The main paper states the assumptions for the finite-cycle and population results, and the appendix provides complete proofs for the additive-invariant contrast, loss invariance, bilinear factorization, exact-marginal interaction shifts, first-order OE transfer, and spectral bottleneck result.  
	
	\item {\bf Experimental result reproducibility}  
	\item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The paper describes the datasets, cycle construction rules, model classes, metrics, train/validation/test splits, seeds, and main hyperparameters. The reproducibility statement says that code, construction scripts, logs, filters, seeds, model definitions, and optimization details are included in the supplementary material.  
	
	\item {\bf Open access to data and code}  
	\item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The paper uses public datasets and states that experimental code, benchmark construction code, logs, seed configurations, filters, model definitions, and optimization details are provided in the supplementary material.  
	
	\item {\bf Experimental setting/details}  
	\item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The experiments section and appendix specify the datasets, construction filters, exact-cycle metrics, CLIP ViT-B/32 features, bilinear rank settings, seeds, number of train/validation/test cycles, epochs, batch size, learning rate, and weight decay.  
	
	\item {\bf Experiment statistical significance}  
	\item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The main tables report mean \(\pm\) standard deviation for multi-seed experiments and probes where variability is measured. Deterministic exact-cycle audits, such as additive audits with identical marginals, are reported as exact chance values when applicable.  
	
	\item {\bf Experiments compute resources}  
	\item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The reproducibility statement reports the hardware used: one NVIDIA V100 GPU with 32GB memory, an Intel Xeon Gold 6248 CPU at 2.5GHz with 20 cores, 256GB DDR4 RAM, and NVMe SSD storage. The paper also reports the main training configuration for the COCO shortcut OE stress test.  
	
	\item {\bf Code of ethics}  
	\item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The work uses public benchmark datasets and pretrained representations, does not involve human subjects or private data collection, and is intended as an evaluation and diagnostic method for improving reliability.  
	
	\item {\bf Broader impacts}  
	\item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The appendix includes a Broader Impact section discussing the positive role of shortcut-audited relational evaluation and noting that cycle accuracy should not be interpreted as a safety certificate or proof of full semantic understanding.  
	
	\item {\bf Safeguards}  
	\item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?  
	\item[] Answer: \answerNA{}.  
	\item[] Justification: The paper does not release a high-risk pretrained model, image generator, language model, or newly scraped dataset. It provides evaluation code and derived benchmark construction scripts based on public datasets.  
	
	\item {\bf Licenses for existing assets}  
	\item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The paper cites the original sources for GQA, MSCOCO, and CLIP, and uses these public assets for evaluation and feature extraction. License and access information for the assets is documented with the supplementary release materials.  
	
	\item {\bf New assets}  
	\item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?  
	\item[] Answer: \answerYes{}.  
	\item[] Justification: The paper introduces cycle construction code and exact-cycle evaluation splits/filters. The construction rules, validity checks, marginal audits, and reproducibility details are described in the main paper and appendix, with code and logs included in the supplementary material.  
	
	\item {\bf Crowdsourcing and research with human subjects}  
	\item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?  
	\item[] Answer: \answerNA{}.  
	\item[] Justification: The paper does not involve crowdsourcing experiments or research with human subjects.  
	
	\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}  
	\item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?  
	\item[] Answer: \answerNA{}.  
	\item[] Justification: The paper does not involve human subjects, crowdsourcing, or collection of participant data.  
	
	\item {\bf Declaration of LLM usage}  
	\item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.  
	\item[] Answer: \answerNA{}.  
	\item[] Justification: The core method does not use LLMs as an important, original, or non-standard component. The paper studies image-caption scoring with CLIP-like representations, cycle construction, and bilinear probes.  
	
\end{enumerate}  

